Constant Acceleration Flow

Rectified flow and reflow procedures have significantly advanced fast generation by progressively straightening ordinary differential equation (ODE) flows. They operate under the assumption that image and noise pairs, known as couplings, can be approximated by straight trajectories with constant velocity. However, we observe that modeling with constant velocity and using reflow procedures have limitations in accurately learning straight trajectories between pairs, resulting in suboptimal performance in few-step generation. To address these limitations, we introduce Constant Acceleration Flow (CAF), a novel framework based on a simple constant acceleration equation. CAF introduces acceleration as an additional learnable variable, allowing for more expressive and accurate estimation of the ODE flow. Moreover, we propose two techniques to further improve estimation accuracy: initial velocity conditioning for the acceleration model and a reflow process for the initial velocity. Our comprehensive studies on toy datasets, CIFAR-10, and ImageNet 64x64 demonstrate that CAF outperforms state-of-the-art baselines for one-step generation. We also show that CAF dramatically improves few-step coupling preservation and inversion over Rectified flow. Code is available at \href{https://github.com/mlvlab/CAF}{https://github.com/mlvlab/CAF}.

==> figures/two_dot_flow2_a.tex <==
\begin{figure}[t]
        \centering
        \includegraphics[width=0.95\columnwidth]{./figures/main_accuracy4.pdf}
    \caption{\textbf{Coupling preservation.} 
    } 
    \label{fig:coupling_prev_qual}
\end{figure}



==> figures/two_dot_flow2_b.tex <==
\begin{figure}[t]
        \centering
        \includegraphics[width=0.65\columnwidth]{./figures/toy_interpolation.pdf}
    \caption{\textbf{Visualization of coupling preservation on 2D synthetic example.} We plot the sampling trajectories of RF and CAF (Ours) during the training, using 2D synthetic data pairs where their interpolation paths $\mathcal{I}$ are crossed. Due to the flow crossing, RF \textit{rewires} the coupling, whereas CAF \textit{preserves} the coupling of training data.
    }
    \label{fig:coupling_prev_synthe}
\end{figure}



==> tables/ex.tex <==
\begin{table}[t]
 \resizebox{.95\linewidth}{!}{
	\centering
	\begin{tabular}{lcccc}
		\toprule
		\multirow{2}{*}{Model} & \multirow{2}{*}{NFE} & \multicolumn{2}{c}{Unconditional} & Conditional \\\cmidrule(lr){3-4}\cmidrule{5-5}
  & & FID$\downarrow$ & NLL$\downarrow$ & FID$\downarrow$ \\\midrule
            \multicolumn{5}{l}{\textbf{Diffusion Models -- Distillation Sampling}}\\
            % KD & 1 & 9.36 & \xmark & - \\
            % DFNO & 1 & 3.78 & \xmark & - \\
            DFNO & 1 & 3.78 & - & - \\
            2-Rectified Flow & 1 & 4.85 & \xmark & - \\
            PD & 1 & 9.12 & \xmark & - \\
            CD (official report) & 1 & 3.55 & \xmark & - \\
            CD (retrained) & 1 & 10.53 & \xmark & - \\
            CD + GAN & 1 & 2.65 & \xmark & - \\
            \cc{15}CTM~(Ours) & \cc{15}1 & \cc{15}\underline{1.98} & \cc{15}\textbf{2.43} & \cc{15}\underline{1.73} \\\cdashlinelr{1-5}%
            PD & 2 & 4.51 & - & - \\
            \cc{15}CTM~(Ours) & \cc{15}2 & \cc{15}\textbf{1.87} & \cc{15}\textbf{2.43} & \cc{15}\textbf{1.63} \\\midrule
            \multicolumn{5}{l}{\textbf{Models without Pre-trained DM -- Direct Generation}}\\
            CT & 1 & 8.70 & \xmark & - \\
            \cc{15}CTM~(Ours) & \cc{15}1 & \cc{15}2.39 & \cc{15}- & \cc{15}- \\
            \bottomrule
	\end{tabular}}
\end{table}



% \begin{table}[t]
% \vskip -0.2in
% 	\scriptsize
%  \caption[Performance comparisons on CIFAR-10.]{Performance comparisons on CIFAR-10}
%  \label{tab:cifar10_baseline}
%  \vskip -0.05in
%  \resizebox{.95\linewidth}{!}{
% 	\centering
% 	\begin{tabular}{lcccc}
% 		\toprule
% 		\multirow{2}{*}{Model} & \multirow{2}{*}{NFE} & \multicolumn{2}{c}{Unconditional} & Conditional \\\cmidrule(lr){3-4}\cmidrule{5-5}
%   & & FID$\downarrow$ & NLL$\downarrow$ & FID$\downarrow$ \\\midrule
%             \multicolumn{5}{l}{\textbf{GAN Models}}\\
%             BigGAN & 1 & 8.51 & \xmark & - \\
%             StyleGAN-Ada & 1 & 2.92 & \xmark & 2.42 \\
%             StyleGAN-D2D & 1 & - & \xmark & 2.26 \\
%             StyleGAN-XL & 1 & - & \xmark & 1.85 \\
%             \midrule
%             \multicolumn{5}{l}{\textbf{Diffusion Models -- Score-based Sampling}}\\
%             DDPM & 1000 & 3.17 & 3.75 & - \\
%             \multirow{2}{*}{DDIM} & 100 & 4.16 & - & - \\
%             & 10 & 13.36 & - & - \\
%             Score SDE & 2000 & 2.20 & 3.45 & - \\
%             VDM & 1000 & 7.41 & \underline{2.49} & - \\
%             LSGM & 138 & 2.10 & 3.43 & - \\
%             EDM & 35 & 2.01 & 2.56 & 1.82 \\\midrule
%             \multicolumn{5}{l}{\textbf{Diffusion Models -- Distillation Sampling}}\\%\cdashlinelr{1-7}
%             KD & 1 & 9.36 & \xmark & - \\
%             DFNO & 1 & 3.78 & \xmark & - \\
%             2-Rectified Flow & 1 & 4.85 & \xmark & - \\
%             PD & 1 & 9.12 & \xmark & - \\
%             CD (official report) & 1 & 3.55 & \xmark & - \\%\cdashlinelr{1-5}
%             CD (retrained) & 1 & 10.53 & \xmark & - \\
%             CD + GAN & 1 & 2.65 & \xmark & - \\
%             \cc{15}CTM~(Ours) & \cc{15}1 & \cc{15}\underline{1.98} & \cc{15}\textbf{2.43} & \cc{15}\underline{1.73} \\\cdashlinelr{1-5}%\cmidrule(lr){1-2}%\cdashlinelr{1-5}
%             %\multicolumn{5}{l}{\textbf{Distillation Models (NFE 2)}}\\
%             PD & 2 & 4.51 & - & - \\
%             CD & 2 & 2.93 & - & - \\
%             \cc{15}CTM~(Ours) & \cc{15}2 & \cc{15}\textbf{1.87} & \cc{15}\textbf{2.43} & \cc{15}\textbf{1.63} \\\midrule
%             \multicolumn{5}{l}{\textbf{Models without Pre-trained DM -- Direct Generation}}\\
%             CT & 1 & 8.70 & \xmark & - \\
%             \cc{15}CTM~(Ours) & \cc{15}1 & \cc{15}2.39 & \cc{15}- & \cc{15}- \\
%             \bottomrule
% 	\end{tabular}}
% \end{table}
